NeuroLogic Decoding: (Un)supervised Neural Text Generation with Predicate Logic Constraints

Conditional text generation often requires lexical constraints, i.e., which words should or shouldn't be included in the output text. While the dominant recipe for conditional text generation has been large-scale pretrained language models that are finetuned on the task-specific training data, such models do not learn to follow the underlying constraints reliably, even when supervised with large amounts of task-specific examples. We propose NeuroLogic Decoding, a simple yet effective algorithm that enables neural language models -- supervised or not -- to generate fluent text while satisfying complex lexical constraints. Our approach is powerful yet efficient. It handles any set of lexical constraints that is expressible under predicate logic, while its asymptotic runtime is equivalent to conventional beam search. Empirical results on four benchmarks show that NeuroLogic Decoding outperforms previous approaches, including algorithms that handle a subset of our constraints. Moreover, we find that unsupervised models with NeuroLogic Decoding often outperform supervised models with conventional decoding, even when the latter is based on considerably larger networks. Our results suggest the limit of large-scale neural networks for fine-grained controllable generation and the promise of inference-time algorithms.

==> fig/c_example.tex <==
\begin{table*}[t]
\footnotesize
    \centering
    \scalebox{.95}{ 
    \begin{tabular}{c|l}
     \toprule

    \rowcolor[gray]{0.90}  \textbf{Constraint} & \hspace{25 mm} \textbf{Description}\\ 
      
\midrule
$ D(\textnormal{Hilton Hotels}) \land D(\textnormal{address}) \land D(\textnormal{phone number}) $ & Generate a response to a user’s query that contains the required \\ &  contact information. \\
 \midrule
   $\big(D(\textnormal{Harry}) \land D(\textnormal{Hermione})\big) \lor \big(D(\textnormal{Harry}) \land D(\textnormal{Ron})\big) $ & Generate a summary for a book chapter that must mention at  \\
   
   $\lor \big(D(\textnormal{Hermione}) \land D(\textnormal{Ron})\big)$  & least two of the three main characters.
\\ 
\midrule
$\big(\neg D(H_2O_2) \lor \neg D(Na) \big) \lor \big(D(H_2O_2) \land D(Na) \land D(N_2)\big)$ & Generate instructions for chemical experiments, if $H_2O_2$ and $Na$
 \\ & are used together, $N_2$ must be used to prevent an explosion.
\\
\midrule
$ D(\textnormal{noodle}) \land \neg D(\textnormal{oil}) \land \big(D(\textnormal{beef}) \lor D(\textnormal{chicken}) \lor \ldots \big)$ & Generate an oil-free chow-mein recipe that uses at least one \\ 

$\land \> \big(D(\textnormal{broccoli}) \lor D(\textnormal{lettuce}) \lor \ldots \big) $ &  type of protein and one type of vegetable. 
 \\
    \bottomrule
    \end{tabular}}
    \caption{Examples of logical lexical constraints. %\rowan{highlight or emphasize that rows 2-4 are NOT POSSIBLE UNDER PRIOR WORK, while row 1 is} \peter{Could we combine this with table 1? Give increasingly difficult constraints and which models can cover them...}
    }  % 
    \label{tab:c_examples}
\end{table*}


==> fig/related_word.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \scalebox{0.95}{ 
    \begin{tabular}{c|c|c}
     \toprule

     \rowcolor[gray]{0.90} \textbf{Method} & \textbf{Expressiveness} &  \textbf{Runtime}  \\ 
      \midrule
     CBS & $\forall S^i \in S, \:\: \exists w \in S^i, \: w \textnormal{ in }\textbf{y}$ & $O(Nk2^C)$ \\
\midrule
     GBS & \multirow{4}{*}{$\forall w \in S \: w \textnormal{ in }\textbf{y} $} & $O(NkC)$  \\
\cmidrule{1-1} \cmidrule{3-3}
 \citeauthor{post-vilar-2018-fast} &&$O(Nk)$  \\
\cmidrule{1-1} \cmidrule{3-3}
 \citeauthor{hu-etal-2019-improved} & &$O(Nk)$  \\
\cmidrule{1-1} \cmidrule{3-3}
 CGMH & & $O(N)$ \\
 \midrule
  \textsc{NeuroLogic} & \textnormal{any logical formula}& $O(Nk)$ \\
    \bottomrule
    \end{tabular}}
    \caption{Comparison of previous work on lexical constrained decoding (given constraint set S, sentence length N, beam size k, and constraint count C. Our proposed \method~is significantly more expressive versus prior work -- allowing any predicate logic formula -- expressed has an equivalent asymptotic runtime as beam search.) 
    }  % 
    \label{tab:c_examples}
\end{table}


==> fig/result_caption.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{|c|c|}
     \toprule

Model &  BLUE \\ 
\midrule
Neural Naturalist & 0.24  \\
\midrule
Neural Naturalist + Oracle Constraint & 0.27  \\
    \bottomrule
    
    \end{tabular}
    \caption{results of find-grained image captioning}  % 
    \label{tab:c_examples}
\end{table*}

==> fig/result_comGen.tex <==
\begin{table*}[t]
\footnotesize
    \centering
    \begin{tabular}{c|c c|c c|c|c c|c}
     \toprule

\textbf{Model / Metrics} &  \multicolumn{2}{c}{\textbf{ROUGE-2/L}} &\multicolumn{2}{c}{\textbf{BLEU-3/4}}  &\textbf{METEOR} &\multicolumn{2}{c}{\textbf{CIDEr} \textbf{SPICE}} &\textbf{Coverage}\\ 
\midrule
\rowcolor[gray]{0.95} \multicolumn{9}{l}{\textit{Without Constrained Decoding}} \\ \midrule
GPT-2 \cite{radford2019language} &19.16 &40.33 & 34.2& 24.7&27.6 &13.38 &27.1  & 82.21 \\
BERT-Gen \cite{radford2019language} &20.85& 42.4&37.5 &27 &29.5 &14.85 &29.8 & 89.09 \\
UniLM\cite{radford2019language} &23.31 &44.34 &40.6 &29.9 &30.1 &15.46 &30.6 &90.51 \\
UniLM-v2  \cite{radford2019language} & 21.78&43.5 &39.2 &28.3 &30.6 &15.62 &30.8 &92.84 \\
BART  \cite{radford2019language} &23.03 &43.27 &39.9 & 29.1& 30.4& 15.18&30.6 &94.98 \\
T5-Base  \cite{radford2019language} & 17.62& 38.09 & 22.5 & 16.1 & 21.5& 8.95&22.4 &70.66 \\
T5-Large  \cite{radford2019language} & 22.61&43.89 & 36.6& 26.9& 28.9& 14.31&29.5 &89.72 \\ \midrule
\rowcolor[gray]{0.95} \multicolumn{9}{l}{\textit{With Our Constrained Decoding}} \\ \midrule

GPT-2 \cite{radford2019language} &20.96 & 42.79 & 36.7 &26.7 &30.2 &14.74 &30.3 &97.7 \\
BERT-Gen \cite{radford2019language} &22 &43.83 &38.9 & 28.2& 30.9&15.53 &31.4 &97.31 \\
UniLM\cite{radford2019language} &24.31 &45.75 &42.8 &31.5 &31.7 &16.61 &32.5 &97.77 \\
UniLM-v2  \cite{radford2019language} &22.29 & 44.21& 39.5 &28.5 & 31.3& 16.78&31.1 &97.86 \\
BART  \cite{radford2019language} & 23.98& 44.67&41.3 &30.6 &31 &15.89 &31 &98.68 \\
T5-Base  \cite{radford2019language} & 20.06&42 &29.8 &20.5 &26.9 & 12.22&26.9 &97.74 \\
T5-Large  \cite{radford2019language} & 23.14& 44.79& 38.5&28.1 &30.7 &15.48 &30.8 &98.48 \\ \midrule


\rowcolor[gray]{0.95} \multicolumn{9}{l}{\textit{Other Decoding Strategy}} \\ \midrule
UniLM + greedy &21.4 &42.1 &36.2 & 25.7&29.5 &13.82 &29.9 &90.49\\
UniLM + top-k &20.27 & 41.26& 34.4&24.4 &28.8 &13.35 &29.2 &89.68\\
UniLM + top-p &21.13 &41.92 &36 &25.7 &29.3 &13.73 &29.8 &90.09\\ \midrule
UniLM + \cite{hokamp-liu-2017-lexically} & 18.97 & 41.04 & 30.8& 21.4 & 27.8 & 12.49 & 27.9& 97.23\\
UniLM + \cite{post-vilar-2018-fast}&19.53 & 41.31&30.6 &21.3 &27.8 &12.18 &27.4 &97.18 \\
UniLM + \cite{hu-etal-2019-improved}&18.04 &40.42 &28.7 &19.6 &27.0 &11.79 &26.8 &96.82 \\\midrule
\rowcolor[gray]{0.95} \multicolumn{9}{l}{\textit{Zero Shot}} \\ \midrule
GPT \cite{Radford2018ImprovingLU} & 20.39 &42.15 &27.1 &17.6  &29 &11.81 &28.4 &97.54 \\
GPT2 \cite{radford2019language} &20.08 &42.18 &35.3 &24.3 &30.5 &13.53 &29 &94.97 \\
CTRL & 21.96 &43.66 &35.4 &24.3  &30.4 &13.78 &30.3 &97.79 \\\midrule
\rowcolor[gray]{0.95} \multicolumn{9}{l}{\textit{Zero Shot (After Language Domain Adaption)}} \\ \midrule
GPT2 \cite{radford2019language} & 22.09&43.47 &39.3 &27.9  &32.3 &14.76 &31.2 &95.96 \\
    \bottomrule
    
    \end{tabular}
    \caption{Experimental results of different methods and decoding strategy on the COMMONGEN test set.  The best models are bold and second best ones are underlined within each metric.\ronan{Impressive table ;) Still wondering if we should have results \emph{with and without constrained decoding} side by side, for easier comparison.}}  % 
    \label{tab:comGen_result}
\end{table*}

==> fig/result_comGen_model_2.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{6pt}
\footnotesize
    \centering
    \begin{tabular}{l|c|c c|c|c c|c}
     \toprule
\rowcolor[gray]{0.90} \textbf{\hspace{8pt}Model} &  \multicolumn{1}{c|}{\textbf{ROUGE - L}} &  \multicolumn{2}{c|}{\textbf{BLEU - 3 \& 4}}  & \textbf{METEOR}  &\multicolumn{2}{c|}{\textbf{CIDEr}   \hspace{15pt} \textbf{SPICE}} &\textbf{Coverage}\\ 
\midrule
GPT-2  %&19.2 $\rightarrow$ 21.0
&40.3 $\rightarrow$ 43.3&34.2 $\rightarrow$ 38.1&24.7 $\rightarrow$ 27.9&27.6 $\rightarrow$ 30.7&13.4 $\rightarrow$ 15.1 &27.1 $\rightarrow$ 30.9&82.2 $\rightarrow$ 97.5\\
UniLM (fas)%&23.3 $\rightarrow$ \textbf{24.3}
&44.3 $\rightarrow$ \textbf{46.1}&40.6 $\rightarrow$ \textbf{43.3}&29.9 $\rightarrow$ \textbf{32.1}&30.1 $\rightarrow$ \textbf{31.6}&15.5 $\rightarrow$ \underline{16.7}&30.6 $\rightarrow$ \textbf{32.5}&90.5 $\rightarrow$ 97.8\\
UniLM %&23.3 $\rightarrow$ \textbf{24.3}
&44.3 $\rightarrow$ \textbf{46.1}&40.6 $\rightarrow$ \textbf{43.5}&29.9 $\rightarrow$ \textbf{32.3}&30.1 $\rightarrow$ \textbf{32.0}&15.5 $\rightarrow$ \underline{16.8}&30.6 $\rightarrow$ \textbf{32.5}&90.5 $\rightarrow$ 98.5\\
    \bottomrule
    
    \end{tabular}
    \caption{with heuristic \ximing{unfortunately other row is still running}
    }  % 
    \label{tab:comGen_result_model_v2}
\end{table*}

==> fig/result_recipe.tex <==
\newcolumntype{x}[1]{%
>{\centering\hspace{0pt}}p{#1}}%

\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{5pt}
    \centering


    \begin{tabular}{c|x{0.97cm} c|x{0.77cm} c| c |c|c|c}
     \toprule

\rowcolor[gray]{0.90}\textbf{Decoding Method}  &  \multicolumn{2}{c|}{\textbf{ROUGE-2/L}} &  \multicolumn{2}{c|}{\textbf{BLEU-3/4}}  & \textbf{METEOR} &\textbf{CIDEr}&\textbf{Coverage}&\textbf{Extra}\\ 
\midrule
Top-k Sampling &12.6 & 27.5& 15.2&9.5 &19.2 &3.0 &84.8 &16.0\\
Top-p Sampling &13.9 &28.7 &\underline{17.6} &11.7 &19.4 &\underline{3.2} &86.4 &15.4\\
Beam Search& \underline{15.2} &\underline{29.4} &17.4 & \underline{12.0}&\underline{19.7} &\underline{3.2} &86.5 &14.3\\\midrule
\citeauthor{post-vilar-2018-fast}&11.4 & 26.1&13.6 &8.8 &16.5 &2.2 &\underline{89.6} &1.15 \\
\citeauthor{hu-etal-2019-improved}&11.4 &26.1 &13.6 &8.8 &16.5 &2.2 &\underline{89.6} &\underline{1.13} \\
\midrule
\textsc{NeuroLogic} &\textbf{18.3}&\textbf{32.1}&\textbf{19.5}&\textbf{13.8}&\textbf{19.8}&\textbf{4.7}&\textbf{95.8}&\textbf{0.6}\\
    \bottomrule
    \end{tabular}
     \caption{Experimental results of different decoding methods with RecipeGPT on the Recipe1M+ test set. \emph{Coverage} indicates the average percentage of ingredients that are covered in the generated recipe, while \emph{Extra} corresponds to the average ratio of extra/hallucinated ingredients over the number of given ingredients.} 
    \label{tab:result_recipe}
\end{table*}

==> fig/result_zero_shot.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|p{2cm}|p{2.2cm}}
     \toprule

      \textbf{Model} & \% semantically valid &\% commonsense valid\\ 
 \midrule
   GPT & - & - \\ 
   GPT-2 & - & - \\ 
   CTRL & - & - \\
   Transformer-XL & - & - \\
    \bottomrule
    \end{tabular}
    \caption{Human Evaluation performance For Zero-shot C{\small OMMON}G{\small EN}}  % 
    \label{tab:zero_result}
\end{table}

==> fig/zero_shot_comGen.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{p{3.5cm}|p{12cm}}
     \toprule

 \hspace{8 mm} \textbf{Concept} & \hspace{35 mm} \textbf{Generation}\\ 
 \midrule
   run team field drill &  The team is happy be in 2016's preseason drill, where it is possible to watch some of the best teams from around the world in the field.\\ 
\midrule

  catch frisbee dog throw &  The dog catches the frisbee the man throws.\\ 
  
  \midrule
  
 food table sit front & The person sits silently in front of table with his hands clasped as he waits for the food to serve.\\
  
  \midrule
stage perform routine music & The people perform music and dance with us. It's not the routine we’ll do on stage.\\
  \midrule
put lipstick talk lip    &  The girl puts lipstick on her lips. I take it that she's just taking it all in. \\
    \midrule
    
wipe open nose tissue pack & The worker opens a pack of tissue and wipes his nose with that.\\
    \bottomrule
    
    \end{tabular}
    \caption{Examples of zero-shot comGen generation}  % 
    \label{tab:zero_com}
\end{table*}

==> section_v2/2_background_v2.tex <==
%\input{fig/related_word}
%\input{fig/constraint_method_table}

\section{Background $\lor$ Related Work}
Today, the dominant approaches for conditional text generation -- generate an output sequence $\mathbf{y}$ given an input sequence $\textbf{x}$ -- are large pretrained left-to-right language models that are then finetuned on a dataset of examples ($\textbf{x}$, $\textbf{y}$). These models for generation are typically trained to maximize the conditional probability $P_\theta(\textbf{y}|\textbf{x})$, yet how to best \emph{decode} from these models is a challenge.

%The two main approaches for decoding today involve \emph{sampling from} or \emph{maximizing} $P_\theta(\textbf{y}|\textbf{x})$. Analysis suggests that maximization-based approaches -- like much of the past work in constrained decoding -- work particularly well for closed-ended conditional generation \cite{holtzman2019curious}. The vast search space of natural language makes exact maximization infeasible, so approximations such as beam search \cite{Och2004TheAT} are frequently used. 

%yet the vast search space of natural language renders exact maximization infeasible. Beam search \cite{Och2004TheAT} is an effective local search algorithm for finding approximately-optimal solutions and has become the de-facto choice for generating sequences from conditional neural language models.


% Sequence generation can be viewed as an optimization problem. The optimal output sequence $\hat{\textbf{y}}$ given input \textbf{x} is the one that maximizes the conditional probability $P_\theta(\textbf{y}|\textbf{x})$ parameterized by a model $\theta$
% \[\hat{\textbf{y}} = \arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\]

% Beam search \cite{Och2004TheAT} is an effective local search algorithm for finding approximately-optimal solution and has become the de-facto choice for generating sequences from conditional neural language models.
% Sequence generation with lexical constraints can be viewed as a \textit{constrained} optimization problem, where the output space is restricted to only those sequences that satisfy the given constraints. We formalize the notation of logical constraints in section \ref{section: notation}, and present our proposed algorithm to find approximately-optimal solutions for constrained optimization in section \ref{section: algo}.

% The observation that language models frequently veer off track has led to several proposed decoding algorithms that a
\subsection{Prior Decoding Approaches}
The observation that language models -- especially the non-pretrained ones of the past -- frequently violate important constraints has led to several approaches for constrained decoding, which we discuss below. There are a few key desiderata that we want out of such a decoding algorithm:
\begin{enumerate}[wide, labelwidth=!,listparindent=0pt, labelindent=0pt,noitemsep,topsep=0pt,parsep=2pt,leftmargin =*,label=\textbf{\alph*})]
    \item \textbf{Expressivity.} The algorithm should be able to handle a variety of complex and compositional lexical constraints. %, ideally both positive and negative.
    \item \textbf{Runtime.} The algorithm should be reasonably fast. 
    %The most expensive operation during decoding is the number of calls of the LM (in scoring the probability of next tokens), which we can use to compare the asymptotic runtime between approaches. 
    Relevant terms can include the length of the sequence $N$, the number of beam-search beams $k$, and the number of constraints $C$.
    \item \textbf{Language quality.} The algorithm should generate fluent and coherent language. %, without an exceptionally low conditional probability under the generator.
\end{enumerate}

\noindent
Earlier approaches, which we discuss below and in Table~\ref{tab:constraint_method_table}, exclusively handle tasks with \emph{positive constraints} where a sequence of at most length $N$ must be generated, while containing a set of $C$ required words (or clauses of words). However, for the tasks we study in this paper, many of the helpful constraints are negative, often prohibiting a long list of irrelevant words that we should not use. This makes minimal dependence on $C$ paramount. As such, we group approaches by their runtime in the number of constraints $C$.
\subsubsection{An approach exponential in $C$: CBS}
% \subsection{Beam Search-Based Approaches}
% \paragraph{Beam search with finite state machines:}
% \citet{anderson-etal-2017-guided} proposed constrained beam search (\textbf{CBS}), which takes sets of constraint words and aim to generate sequences containing at least one word from each set. CBS leverage state of finite-state machine (FSM) to mark completed subsets of the constraint sets. For $C$ constraint sets, $2^C$ state is required. For each state in the FSM, a search beam with size $k$ is maintained. At each time step, all $2^Ck$ hypothesises are expanded, and each beam is updated by retaining the $k$ most likely candidates whose next-word extension transit its previous hypothesis to the state corresponding to this beam. The accepting state is where all constraints are completed. Due to its massive exploration of search space, it's likely to find approximately optimal sequence under constraints. However, because of its exponential complexity $O(Nk2^C)$, it's infeasible for large-scale language generation with multiple constraints. 
\citet{anderson-etal-2017-guided} propose constrained beam search (\textbf{CBS}), where constraint satisfaction is recorded using a finite-state machine with $2^{C}$ states (one for each possible assignment of completed constraints). Beam search is then done over all states with $k$ candidates per state; candidates move from one state to another. In the end, we retrieve the best-scoring sequence from the `all-constraints-satisfied' state. This method suffers from an exponential complexity of $O(Nk2^C)$, making it infeasible for language generation with many constraints. 

\subsubsection{An approach linear in $C$: GBS}
\citet{hokamp-liu-2017-lexically} propose grid beam search (GBS), which groups together hypotheses by the number of constraints that they satisfy. This results in $C+1$ separate groups altogether. Each group stores at most $k$ candidates that are expanded at each timestep; these candidates move groups accordingly based on the number of constraints they satisfy. Though GBS has a faster runtime of $O(NkC)$, the choice of data structure also can hurt language quality: the decoder has limited capability to generate sequences where the constraints are filled in a non-greedy order.

\subsubsection{Approaches without explicit dependence on $C$}
\paragraph{Dynamic beams for GBS}
\citet{post-vilar-2018-fast} propose an approach to reduce GBS's explicit dependence on $C$. Beam search is done over a single beam, with the slots of this beam dynamically allocated over the $C+1$ groups explicitly used by GBS. This approach was made GPU-efficient by \citet{hu-etal-2019-improved}. Still, the language quality issue of GBS remains, and can be worse in practice as fewer hypotheses are considered at each step.

% proposed dynamic beam allocation to reduce the runtime of GBS from linear to constant $O(Nk)$ with respect to number of constraints. Instead of maintaining $C + 1$ banks of beams, \citeauthor{post-vilar-2018-fast} maintain a single beam of size $k$ and dynamically allocate the slots of this beam across the constraint banks at each time step. \citet{hu-etal-2019-improved} vectorized dynamic beam allocation to enable batching and GPU computing, which efficiently speedup the algorithm in practice.  
  
\paragraph{Local editing with sampling}
\citet{miao2019cgmh} propose Constrained Generation by Metropolis-Hastings sampling (\textbf{CGMH}). This approach begins a sentence by inserting all positive-constraint keywords, in random order. Operations are then randomly sampled to replace, insert, or delete words from the sentence; the probabilities are computed on top of the language model. This approach thus has a runtime (in terms of number of generator calls) independent of the number of constraints; yet in practice it can involve repeated deletions and insertions, reducing efficiency. Moreover, generation quality is highly sensitive to the order of the keywords in the initial state and sampled edits.


% \citet{miao2019cgmh} proposed Constrained Generation by Metropolis-Hastings sampling (\textbf{CGMH}). 
% %framework that uses Metropolis-Hastings sampling for constrained sentence generation. 
% CGMH takes in a set of keywords that require mandatory inclusion as constraints. For sentence generation, each state of the Markov chain is a particular sentence. The initial state is the sequence of keywords placed in random order. The authors design a Markov chain whose stationary distribution is proportional to the language model probability if all constraints are satisfied, $0$ otherwise. To obtain a stationary distribution, the authors leverage MH sampler which first proposes a tentative transition: word-level replacement, insertion, deletion, and accepts or rejects the proposal according an acceptance rate. The acceptance rate is a function of the stationary distribution and proposal distribution to guarantees that MH converges to the desired distribution. However, since CGMH relies on word-level local editing only, the generation quality is very sensitive to the order of keywords in initial state and unlikely to find a globally optimal sentence under given constraints. The runtime of CGMH ($O(N)$) is constant with respect to the number of constraints.

%Due to page limitation, we omit constrained generation methods that require modification to model structure and incompatible with pre-trained language models without re-training.







% , with sequences passing from one 

% which takes sets of constraint words and aim to generate sequences containing at least one word from each set. CBS leverage state of finite-state machine (FSM) to mark completed subsets of the constraint sets. For $C$ constraint sets, $2^C$ state is required. For each state in the FSM, a search beam with size $k$ is maintained. At each time step, all $2^Ck$ hypothesises are expanded, and each beam is updated by retaining the $k$ most likely candidates whose next-word extension transit its previous hypothesis to the state corresponding to this beam. The accepting state is where all constraints are completed. Due to its massive exploration of search space, it's likely to find approximately optimal sequence under constraints. However, because of its exponential complexity $O(Nk2^C)$, it's infeasible for large-scale language generation with multiple constraints. 

% \paragraph{Grid beam search (GBS):}
% \citet{hokamp-liu-2017-lexically} introduced grid beam search (GBS), which groups together hypotheses by the number of constraints that they satisfy. This results in $C+1$ separate groups altogether. Each group stores at most $k$ candidates that are expanded at each timestep; these candidates move groups accordingly based on the number of constraints they satisfy. This is 


% that takes a set of constraint words and aim to generate output containing all constraint words. For $C$ constraints, $C + 1$ separate beams or \emph{banks} are maintained to groups together hypotheses that have generated the same number of the constraints. At each time step, all hypotheses are expanded, and each bank is filled by selecting $k$ most likely candidates whose number of satisfied constraints corresponding to this bank. \ximing{Following sentence: we need a better way to explain why in reality even with simplest all AND constraints, this method still doesn't work} Although GBS reduce to linear complexity $O(NkC)$, organizing hypotheses in terms of the number of satisfied constraints instead of the subset of satisfied constraints limits its capability to explore sequences placing constraint words in different order and find a sequence where the order of constraints is globally optimal, which makes it only applicable in scenario where the semantic of source sentence and target sentence align, like machine translation. 

% \paragraph{Dynamic beams:}
% \citet{post-vilar-2018-fast} proposed dynamic beam allocation to reduce the runtime of GBS from linear to constant $O(Nk)$ with respect to number of constraints. Instead of maintaining $C + 1$ banks of beams, \citeauthor{post-vilar-2018-fast} maintain a single beam of size $k$ and dynamically allocate the slots of this beam across the constraint banks at each time step. \citet{hu-etal-2019-improved} vectorized dynamic beam allocation to enable batching and GPU computing, which efficiently speedup the algorithm in practice.  
  
% \subsection{Sampling Based Method} 
% \paragraph{Local editing with sampling}
% \citet{miao2019cgmh} proposed Constrained Generation by Metropolis-Hastings sampling (\textbf{CGMH}). 
% %framework that uses Metropolis-Hastings sampling for constrained sentence generation. 
% CGMH takes in a set of keywords that require mandatory inclusion as constraints. For sentence generation, each state of the Markov chain is a particular sentence. The initial state is the sequence of keywords placed in random order. The authors design a Markov chain whose stationary distribution is proportional to the language model probability if all constraints are satisfied, $0$ otherwise. To obtain a stationary distribution, the authors leverage MH sampler which first proposes a tentative transition: word-level replacement, insertion, deletion, and accepts or rejects the proposal according an acceptance rate. The acceptance rate is a function of the stationary distribution and proposal distribution to guarantees that MH converges to the desired distribution. However, since CGMH relies on word-level local editing only, the generation quality is very sensitive to the order of keywords in initial state and unlikely to find a globally optimal sentence under given constraints. The runtime of CGMH ($O(N)$) is constant with respect to the number of constraints.

%Due to page limitation, we omit constrained generation methods that require modification to model structure and incompatible with pre-trained language models without re-training.

\subsection{Applications of Lexically Constrained Generation}  
%A lot of study focus on the application of lexical constrained decoding in neural machine translation field. 
Many prior studies on conditional text generation and revision can be viewed as applications of lexically constrained generation. 
Examples include incorporating pre-specified lexical constraints \cite{anderson-etal-2017-guided, post-vilar-2018-fast},  user-provided terminology constraints \cite{hasler-etal-2018-neural, dinu-etal-2019-training}, noisy automatic constraints \cite{li2019neural} into translation output. Another major use case of lexical constrained decoding is paraphrase generation \cite{hu-etal-2019-improved, kajiwara-2019-negative, Hu2019ParaBankMB, miao2019cgmh}, where words in the source sentence that require paraphrasing can be negatively constrained for the output to enforce paraphrasing.
%A typical pipeline is to first identify words in the source sentence requiring paraphrasing, then negatively constrain these words to not appear in the output sequence to force them be paraphrased. 
Another application lies in images captioning for novel scenes or out-of-domain objects \cite{anderson-etal-2017-guided} or image captioning with explicit grounding to objects in the scene  \cite{Ren2015FasterRT, Krause2016TheUE}.
%An advantage of object detectors is they are easier to scale to new concepts.\cite{Ren2015FasterRT, Krause2016TheUE} 
%Lexically constrained decoding enables caption system to leverage such advantage by incorporating detected object tags into caption generation to improve the quality of resulting captions.




==> section_v2/3_model.tex <==
\makeatletter
\newcommand{\stx}[1]{\mathpalette\giusti@stx{#1}}
\newcommand{\giusti@stx}[2]{%
  \mbox{%
    \medmuskip=\thinmuskip
    \thickmuskip=\thinmuskip
    $\m@th#1#2$%
  }%
}
\makeatother
% \input{fig/c_example}
%\input{fig/constraint_method_table}
\section{Our Method: NeuroLogic Decoding}
Our algorithm generalizes past work on lexically constrained generation by modifying beam search to handle richer constraints specified in any predicate logic constraint, while also improving the search efficiency by creating bins within the beam with diverse partial clause satisfactions. %, while yielding high-quality text. 
%Like Beam Search, we search over left-to-right sequences to maximize the conditional probability $P_\theta(\textbf{y}|\textbf{x})$, yet here we introduce machinery enabling these logical constraints to be tracked efficiently, and diversely. % (different ways and orders in which the constraints are satisfied). 
%We formalize the notation of logical constraints and present our proposed algorithm to find approximately-optimal solutions for constrained optimization in section \ref{section: algo}.

% Sequence generation can be viewed as an optimization problem. The optimal output sequence $\hat{\textbf{y}}$ given input \textbf{x} is the one that maximizes the conditional probability $P_\theta(\textbf{y}|\textbf{x})$ parameterized by a model $\theta$
% \[\hat{\textbf{y}} = \arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\]

% Beam search \cite{Och2004TheAT} is an effective local search algorithm for finding approximately-optimal solution and has become the de-facto choice for generating sequences from conditional neural language models.
% Sequence generation with lexical constraints can be viewed as a \textit{constrained} optimization problem, where the output space is restricted to only those sequences that satisfy the given constraints. We formalize the notation of logical constraints in section \ref{section: notation}, and present our proposed algorithm to find approximately-optimal solutions for constrained optimization in section \ref{section: algo}.

%\subsection{Notation} \label{section: notation}
%Predicate $D(\textbf{c})$ is a boolean function indicating whether a word or phrase $\textbf{c}$ occurs in a sequence $\textbf{y}$. $D(\textbf{c})$ will be true iff \textbf{y} contains $\textbf{c}$. Formally, 
%\begin{align*}
%    &D(\textbf{c}) \equiv \exists \: i, \> \textbf{y}_{i:i+|\textbf{c}|} = \textbf{c}
%\end{align*}
%For instance, enforcing a single positive or negative constraint $\textbf{a}_\textbf{i}$ to be satisfied is equivalent to enforcing literal $D(\textbf{a}_\textbf{i})$ or $\neg D(\textbf{a}_\textbf{i})$ to be true. Two or more single constraints can be connected using any logical operator to form a compound logical constraint $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ to represent arbitrarily complex lexical constraints. Table \ref{tab:c_examples} shows some examples. Previous works, on the other hand, only take constraints in certain form, which limits their expressiveness. 

%Our goal in this work is to find a way to enforce these logical constraints on generation output.
%Formally, we seek an optimal solution $\hat{\textbf{y}}$ for the following constrained optimization problem:
%\begin{align*}
%    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\\
%    &\text{subject to}\\
%    &D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n}) \text{ is true }
% \end{align*}
 
% \ximing{perhaps we will need to find a cleaner way to replace $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ to express compound constraint, thoughts/ideas ? }



\subsection{Algorithm} \label{section: algo}
%\ximing{should we mention all logical form can turn in to CNF, so we can handle everything?}
\method accepts lexical constraints in Conjunctive Normal Form (CNF):
% Thus, it is sufficient to assume that all constraints our algorithm deals with are in CNF. 
% Without loss of generality, we assume that constraints $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ can be expressed in CNF:
\[\big(D_1 \lor D_2 \cdots \lor D_i \big) \land \cdots \land \big(D_k \lor D_{k+1} \cdots \lor D_n \big) \]
where each $D_i$ represents a single positive or negative lexical constraint  $D(\textbf{a}_\textbf{i})$ or $\neg D(\textbf{a}_\textbf{i})$ indicating whether word/phrase $\textbf{a}_\textbf{i}$ is strictly included or omitted (respectively). Any combination of such constraints that are expressible as a predicate logical formula can be converted to CNF, and thus handled by \method. Notationally, we will refer to each individual constraint $D_i$ as a literal, and the disjunction of literals (bracketed AND term, above) as a clause, denoted as $C_j$, with $L$ being the total number of clauses. Our method seeks optimal sequences in which all clauses are satisfied: 

\vspace*{-9mm}
\begin{equation}
    \hat{\textbf{y}} {=} \arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) \hspace{1em}\textrm{where}\hspace{1em} \sum_{i=1}^{L} C_i{=}L
 \end{equation}
Past work on constrained optimization introduces penalties \cite{Fiacco1976SensitivityAF} to approximate the constrained optimization problem with an unconstrained problem. Specifically, by adding a high-cost penalty term for violated constraints:

\vspace*{-5mm}
\begin{align}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) - \alpha' \sum_{i=1}^{L} (1-C_i)
 \end{align}
%where high $\alpha'$ results in significant objective reduction for any violated constraint. 
Intuitively, this objective balances sequence likelihood (term 1) and constraint satisfaction (term 2). 
%We take a related approach, by attempting to find sequences that do well at both term 1 and term 2. 
While exhaustive search is intractable, we use a modified beam search to find approximately-optimal solutions for this objective. At each decoding step, we fill the beam with the most likely (term 1) candidates across a range of values for term 2, allowing a balance of candidates that are likely, and satisfy the most constraints in each beam. In the end, we take the candidates with the most constraints satisfied (term 2), and select the most probable (term 1) one from this group. 
%As a result, we constrain the search space to strings which satisfy given constraints. 
%\ximing{add Dominance Set from Multi-Objective Optimization }

\begin{comment}
\subsubsection{Tracking Clause Satisfaction}
When considering whether a generation hypothesis satisfies some clause $C_i$ during generation, there are fundamentally 3 options. Case 1: if a \textit{positive} constraint $D(\textbf{a}_\textbf{i})$ in the clause is satisfied, the full clause is permanently satisfied by the hypothesis. By definition, the hypothesis contains $\textbf{a}_\textbf{i}$ and further decoding cannot change this. In contrast, if only negative constraints $\neg D(\textbf{a}_\textbf{i})$ are satisfied (case 2), it is possible this clause will become unsatisfied if further decoding produces the word/phrase $\textbf{a}_\textbf{i}$. Finally, case 3 is the simple case in which the clause is not (yet) satisfied.
%
Fundamentally, we only need to keep track of clauses in case 2 or 3, as we know the value of any clause in case 1 for the final generation already. Thus, we only track constraints that appear in a clause in case 2 or 3 for some hypothesis in the beam. 
%For a clause $C_i$, if its satisfaction can not be violated in later decoding step, we say it is \emph{robustly satisfied}. A clause is \emph{robustly satisfied} if and only if at least one of its literals is satisfied positive literal.
%\[ C^i_{\textbf{y}_t} \textnormal { is true} \longrightarrow \forall \> t' > t, \: C^i_{\textbf{y}_{t'}} \textnormal { is true} \]
 %On the other hand, if the satisfaction state of a clause $C_i$ can be violated by later generation, we refer to it as \emph{vulnerably satisfied}. This situation can happen when the clause has one or more satisfied negative literals, but no satisfied positive literal. 

%At each time step for each hypothesis in beam, we keep track of its satisfaction status of literals and clauses. At the beginning when nothing has been generated, all positive literals are unsatisfied and all negative literals are satisfied. A clause will be marked as satisfied once at least one of its literals is satisfied. As decoding proceeds, we only need to keep track of unsatisfied clauses and \emph{vulnerably satisfied} clauses.

To efficiently track the occurrence of a constrained word/phrase as the generation proceeds, we keep track of the matched partial prefix of each literal in the ongoing generation by maintaining a pointer to its token(s). At the beginning, the pointer is set to the head of the literal. At each time step, if the next generated token matches the token of the pointer, we advance the pointer forward, otherwise we set the pointer back to the head of the literal. A special case is when the next generated token does not match the token of the pointer but matches another token of the literal, in which case, we set the pointer after the longest prefix of the literal that is also a suffix of the current generation. If the pointer reaches the end, this constraint has been generated in the decoded sentence, and we'll mark this literal as satisfied or unsatisfied depending on whether it's positive or negative, and update its clause status accordingly.
\end{comment}

\subsubsection{Beam Search with Bins with Diverse Partial Satisfaction}

%\peter{Here is the new version}

At each time step, the decoding model generates a distribution over all vocabulary $V$ for $k$ hypotheses in the current beam, resulting in a candidate score matrix of size $k \times |V|$. %Standard beam search fills in beam at time step t + 1 with candidates corresponding to the $k$ best scores. Our method, on the other hand, select $k$ candidates that represent a range of optimality between score and number of satisfied clauses.
%
Along with generating score matrix, we produce a constraint state for each of the $k \times |V|$ new candidate hypotheses $h$, based on the next token considered. We discard any $h$ with unsatisfiable clauses, i.e. any clause with only negative constraints that all appear in $h$, to focus only on candidates that might satisfy all constraints.

Next is selection of a beam of k candidates $h$ for the next decoding step. 
%Here, we aim to balance high decoding score with high number of satisfied constraints, to ensure progress on satisfying constraint clauses, without resulting in degenerate solutions. We achieve this in three ways.
%
First, we filter candidate hypotheses $h$ to those in the top-tier of both satisfied constraints and decoding score. Specifically, we drop any candidates not in the top-$\alpha$ in terms of decoding score, and not in one of the top-$\beta$ bins in terms of number of satisfied clauses. These are adjustable parameters, deciding how diverse a set of candidates to choose the next beam from. 
\begin{comment}
\ximing{change here}
Second, we compute the objective function for remaining candidates following equation (1), with simple algebra, we can rewrite (1) as 
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) + \alpha' \sum_{i=1}^{L} C_i
 \end{align*}
While the objective score is directly intractable, we factorize it into a chain of step-wise objectives. 
\begin{align*}
    \hat{\textbf{y}_t} = &\arg\max_{\textbf{y}_t \in \mathcal{V}}P_\theta(\textbf{y}_t|\textbf{x}, \textbf{y}_{ \leq t-1}) \\ & + \alpha'\cdot P_\theta(
     \prod_{i=1}^{L} C_i = 1 |\textbf{x}, \textbf{y}_{\leq t} )
 \end{align*}

Intuitively, term 2 measure how likely current unsatisfied clause will be satisfied in the future step. For clause containing negative literal, we can guarantee its satisfaction by force exclusion of certain word or phrase. Otherwise, we need "looking ahead" to determine how likely at least one of its literal will appear in the future. Since throughout looking ahead is computationally intractable, we look at the near future with a window size k. In this scenario, we cannot expect all unsatisfied clause will be satisfied in next k step, otherwise it'll result in much shorter sequence that breaks fluency and plausibility. Instead, we're interested in how likely one more clause will be satisfied in next k step. \begin{align*}
&\max_{\{C_i | C_i = 0\}} P_\theta( C_i = 1 |\textbf{x}, \textbf{y}_{\leq t} )\\
=&\max_{\{C_i | C_i = 0\}} \max_{L_i \in C_i}  P_\theta( L_i = 1 |\textbf{x}, \textbf{y}_{\leq t} )\\
=& \max_{\{L_i | L_i \in \{C_i | C_i = 0\}\}} P_\theta( L_i = 1 |\textbf{x}, \textbf{y}_{\leq t} ) \\
=& \max_{\{L_i | L_i \in \{C_i | C_i = 0\}\}} \max_{k'=1}^{k} P_\theta( \textbf{y}_{t + k'} = L_i |\textbf{x}, \textbf{y}_{\leq t} )
 \end{align*}
To compute $P_\theta( \textbf{y}_{t + k'}|\textbf{x}, \textbf{y}_{\leq t}) $ using an autoregressive model, we use greedy decoding to approximate $y_{t: t+k'}$. In non-autoregressive model, we can directly attain this marginalized probability by masking out $y_{t: t+k'}$. 
%Here we're using an estimation of future state to guide exploration. 
\end{comment}

Next, we select the beam ($k$ candidates). 
%We aim to represent a range of natural sentences (i.e. high decoding score) while also encouraging constraint satisfaction, and so will include a range of candidates that optimize for both of these things. We start by binning candidates by set of clauses satisfied. 
To ensure the diversity of partially satisfied constraints, we create bins within the beam by set of clauses satisfied. 
%
We then proceed in rounds of filling the beam, visiting each bin in rotation, until we reach k candidates.
%In each round $j$, we take the $j^{th}$ candidate in each bin, as ranked by decoding score, then fill in the beam from this set in order of decoding score. In the first round, this means taking the top-scored candidate for each unique set of satisfied clauses. By taking one example from each bin (defined by constraint set) we assure that the beam is filled with candidates that satisfy a range of different constraints. By selecting for decoding score, both within each bin and when filling the beam, we prioritize natural and well-formed sentences. Over many steps, this results in high quality hypotheses that satisfy the desired constraints. 
%
In the end, 
we 
%bin by number of clauses satisfied, then
take the highest-scoring hypothesis from the highest-clause bin. %, ensuring the final generation satisfies as many clauses as possible.
Appendix~\ref{ssec:tracking} provides  implementation details on efficient tracking of clause satisfaction.


%\peter{New version above =======}

%At each time step t, the decoder model generates a distribution over all vocabulary $V$ for $k$ hypotheses in current beam, resulting in a candidate score matrix of size $k \times |V|$. Standard beam search fills in beam at time step t + 1 with candidates corresponding to the $k$ best scores. Our method, on the other hand, select $k$ best candidates that's both optimal in score and number of satisfied clauses.

%Along with generating score matrix, we produce advanced constraint state for each candidate by updating the constraint state of its previous hypotheses based on its next-token extension. To ensure progress is made towards satisfying all constraints at the end, we discard the candidates whose next-token extension makes some clause impossible to satisfy in the following decoding step. This situation can happen when some clauses contain only negative literals, and the next-token extension completes the generation of all these negative literals.

%\ximing{top-a, top-B is to tolerate sub-optimal sequence that hit constraints}
%Our next step is to select best candidates that maximizes both sequence score and number of satisfied clauses. If we plot the candidates as points in a coordinate whose x-axis is number of satisfied clauses, and y-axis is sequence score, the optimal candidates are at top-right corner, which corresponds to high sequence score and more satisfied clauses. Following this intuition, We use threshold pruning to reduce candidate set and only keep the ones around top-right. Concretely, we'll remove candidates whose score is not within top-$\alpha$ or whose number of satisfied clauses is not within top-$\beta$, where $\alpha$ and $\beta$ are tunable threshold.

%\ximing{the reason why we need bucket is that generation will pick next unsatisfied constraint with highest likelihood, but that's only local optimal. After consuming a few high likelihood constraints, it might have no proper place to put the rest unsatisfied constraints. A global optimal sentence might start with subsequence with lower likelihood including hard-to-satisfied constraints. We want to keep some sub-optimal subsequence to explore this possibility. In experiments, I found this is very important, that's the exact reason why previous method fails even in all AND cases. } 

%\ximing{once we have the look-ahead heuristic, we can further guarantee local path to next picked constraint is optimal}
%Now, we'll select $k$ item from reduced candidate set to fill in the next beam. We group the candidates into buckets based on satisfied constraint clauses. Then we iteratively pick and remove candidate with highest score within each bucket in a round-robin fashion until all $k$ slot are filled. As a result, we preserve most likely sequence for each set of satisfied clauses in beam. This not only ensure progress is made towards optimizing proposed objective but also encourage exploring candidates which satisfy constraint clauses in different order and address the issue that .

%In the end, we'll select the one with maximum likelihood from finished hypothesises which satisfy maximum number of constraint clauses as the final output. As a result, we end up with the optimal sequence among all strings satisfying given logical constraints.

%Please refer to figure 1 for detailed algorithm

==> section_v2/backups/2_background.tex <==
\section{Related Work}


% \paragraph{Lexical Constrained Decoding} \citet{anderson-etal-2017-guided} extends beam search with a finite state machine marking included subsets of given word set to force the inclusion of selected tag words in the output. Due to its exponential complexity in the number of constraints, it's infeasible for large-scale language generation with multiple constraints. 

%\cite{hokamp-liu-2017-lexically} introduced grid beam search algorithm, which takes a set of constraints which specify certain word(s) must appear or not appear in the output and ensures hypotheses have met all constraints before can be considered completed. \cite{post-vilar-2018-fast} and \cite{hu-etal-2019-improved} improved grid beam search by reducing the time complexity from linear to constant with respect to the number of constraints. 
%Another related approach proposed by \cite{anderson-etal-2017-guided} extended beam search with a finite state machine whose states marked completed subsets of the set of constraints.

 %\cite{hokamp-liu-2017-lexically} introduce grid beam search with linear time complexity that allow the inclusion and exclusion of pre-specified lexical constraints by maintaining 2-dimensional beam. 
 \citet{post-vilar-2018-fast} and \citet{hu-etal-2019-improved} reduces the time complexity to constant by proposing dynamic and vectorized beam allocation with fixed-size beam. The limitation of these approach is that the constraints they handle is either positive or negative, which limit their feasibility in applications with more complex lexical constraints (i.e. morphology in C{\small OMMON}G{\small EN}). 
 
\citet{miao2019cgmh} proposed CGMH framework that uses Metropolis-Hastings sampling for constrained sentence generation. CGMH handles both hard constraints, mandatory inclusion of certain keywords, and soft constraints, requirement of semantic relevance. While hard constraints suffers from the same limitation with method above, soft constraints focus on the semantic similarity at sentences level and lose the controllability over output at lexical level. \citet{li2019neural} proposed a novel framework to handle noisy constraints by adding additional modules to standard Seq2Seq framework. Due to its modification to model structure, it's incompatible with modern pre-trained language models without re-training. 

\paragraph{Applications}  A lot of study focus on the application of lexical constrained decoding in neural machine translation field. Examples includes incorporating pre-specified lexical constraints \cite{anderson-etal-2017-guided, post-vilar-2018-fast},  user-provided terminology constraints \cite{hasler-etal-2018-neural, dinu-etal-2019-training}, noisy automatic constraints \cite{li2019neural} into translation output. Another major usage of lexical constrained decoding is in paraphrase generation. \cite{hu-etal-2019-improved, kajiwara-2019-negative, Hu2019ParaBankMB, miao2019cgmh} A typical pipeline is to first identify words in the source sentence requiring paraphrasing, then negatively constrain these words to not appear in the output sequence to force them be paraphrased. Another application lies in out-of-domain images captioning with novel scenes or objects. \cite{anderson-etal-2017-guided}. An advantage of object detectors is they are easier to scale to new concepts.\cite{Ren2015FasterRT, Krause2016TheUE} Lexical constrained decoding enables caption system to leverage such advantage by incorporating detected object tags into caption generation to improve the quality of resulting captions.




==> section_v2/backups/2_background_v3.tex <==
%\input{fig/related_word}
%\input{fig/constraint_method_table}

\section{Related Work}
\subsection{Prior Decoding Approaches}
There are two main appr
\subsection{Applications of Lexically Constrained Generation}  
%A lot of study focus on the application of lexical constrained decoding in neural machine translation field. 
Many prior studies on conditional text generation and revision can be viewed as applications of lexically constrained generation. 
Examples include incorporating pre-specified lexical constraints \cite{anderson-etal-2017-guided, post-vilar-2018-fast},  user-provided terminology constraints \cite{hasler-etal-2018-neural, dinu-etal-2019-training}, noisy automatic constraints \cite{li2019neural} into translation output. Another major use case of lexical constrained decoding is paraphrase generation \cite{hu-etal-2019-improved, kajiwara-2019-negative, Hu2019ParaBankMB, miao2019cgmh}, where words in the source sentence that require paraphrasing can be negatively constrained for the output to enforce paraphrasing.
%A typical pipeline is to first identify words in the source sentence requiring paraphrasing, then negatively constrain these words to not appear in the output sequence to force them be paraphrased. 
Another application lies in images captioning for novel scenes or out-of-domain objects \cite{anderson-etal-2017-guided} or image captioning with explicit grounding to objects in the scene  \cite{Ren2015FasterRT, Krause2016TheUE}.
%An advantage of object detectors is they are easier to scale to new concepts.\cite{Ren2015FasterRT, Krause2016TheUE} 
%Lexically constrained decoding enables caption system to leverage such advantage by incorporating detected object tags into caption generation to improve the quality of resulting captions.




==> section_v2/backups/3_model_0.tex <==
\makeatletter
\newcommand{\stx}[1]{\mathpalette\giusti@stx{#1}}
\newcommand{\giusti@stx}[2]{%
  \mbox{%
    \medmuskip=\thinmuskip
    \thickmuskip=\thinmuskip
    $\m@th#1#2$%
  }%
}
\makeatother
\input{fig/c_example}
\section{Our Method: NeuroLogic Decoding}
NeuroLogic Decoding generalizes past work to any constraints that can be encoded as a logical formula. It efficiently leverages constraints as prior knowledge to restrict the search space and leads to better generation quality. 

Sequence generation can be viewed as an optimization problem. The optimal output sequence $\hat{\textbf{y}}$ given input \textbf{x} is the one that maximizes the conditional probability $P_\theta(\textbf{y}|\textbf{x})$ parameterized by a model $\theta$
\[\hat{\textbf{y}} = \arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\]

Beam search \cite{Och2004TheAT} is an effective local search algorithm for finding approximately-optimal solution and has become the de-facto choice for sequences decoding with neural language model.

Sequence generation with lexical constraints can be viewed as constrained optimization problem, where output space is restricted to strings satisfying given constraints. We'll give a formal formulation of logical constraints in section \ref{section: notation}, and present proposed algorithm to find approximately-optimal solution via constrained optimization in section \ref{section: algo}

\subsection{Notation} \label{section: notation}
Predicate $D(\textbf{c})$ is a boolean function indicating word or phrase $\textbf{c}$ occurs in sequence $\textbf{y}$. $D(\textbf{c})$ will be true if and only if \textbf{y} contains $\textbf{c}$. Formally, 
\begin{align*}
    &D(\textbf{c}) \equiv \exists \: i, \> \textbf{y}_{i:i+|\textbf{c}|} = \textbf{c}
\end{align*}
For instance, enforcing a single positive or negative constraint $\textbf{c}_\textbf{i}$ to be satisfied is equivalent to enforcing literal $D(\textbf{c}_\textbf{i})$ or $\neg D(\textbf{c}_\textbf{i})$ to be true. Two or more single constraints can be connected using any logical operator to form a compound logical constraint $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ to represent arbitrary complex lexical restrictions. Please refer to Table \ref{tab:c_examples} for some examples. Previous works, on the other hand, only take constraints in certain form, which limits their expressiveness. 

Our goal in this work is to find a way to enforce these logical constraints on generation output.
Formally, we seek an optimal solution $\hat{\textbf{y}}$ for the following constrained optimization problem:
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\\
    &\text{subject to}\\
    &D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n}) \text{ is true }
 \end{align*}

\begin{figure*}[t]
\centering
    \includegraphics[width=1\linewidth]{fig/fig2_v5.pdf}
     \caption{Algorithm of selecting hypothesis to fill in next beam from candidates \rowan{we want to show the following 1. we can use a new constraint that has never been used before-- `Use at least one of X or Y', 2. we can do so without recomputing everything. 3. We want to have diversity in the satisfaction status (allowing for exploration) <- mention this at the beginning of the new sec3 To this, you might not need multiple rows or a multi-clause expression and putting it in natural language could help. For the $\alpha$/$\beta$ constraints maybe use a fake bar graph}
     } 
\end{figure*} 

\subsection{Algorithm} \label{section: algo}
Every logical formula can be equivalently written in conjunctive normal form (CNF). So for any logical constraint $D$, it's guaranteed to find an equivalent logical constraint $D'$ in CNF form. Thus, it's sufficient to assume all constraint our algorithm deals with are CNF. Without loss of generality, assume constraint $D$ take the form:
\[\big(D_1 \lor D_2 \cdots \lor D_i \big) \land \cdots \land \big(D_k \lor D_{k+1} \cdots \lor D_n \big) \]
where each $D_i$ can be either $D(\textbf{c}_\textbf{i})$ or $\neg D(\textbf{c}_\textbf{i})$. We refer $D_i$ as a literal, and a disjunction of literals as a clause, denote as $C_i$. Let $N$ be the number of clauses in $D$.  A clause is marked as satisfied if at least one of its literals are satisfied. A Cl

Our method seeks for optimal sequence in which all clauses are satisfied, formally 
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\\
    &\text{subject to}\\
    & \sum_{i=1}^{N} C_i = N
 \end{align*}
Past work on constrained optimization uses a penalty function method \cite{Fiacco1976SensitivityAF} to approximate the constrained optimization problem with an unconstrained problem. Specifically, by adding a high-cost penalty term to the objective for violation of constraints:
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) - \alpha \Big(\sum_{i=1}^{N} C_i - N \Big)^2
 \end{align*}
Since $\sum_{i=1}^{N} C_i$ takes value in $[0, N]$ and penalty term monotonically increase within this interval, we can equivalently rewrite the objective as 
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) + \alpha' \sum_{i=1}^{N} C_i
 \end{align*}
 \peter{Is there any reason not to just use this second equation directly? i.e. do we need to start with the eqn with the squared penalty?}
Intuitively, this objective aims to optimize both sequence likelihood and number of satisfied clauses. While exhaustive search is intractable due to exponential search space, we use a modified beam search to find approximately-optimal solutions for this objective. At a high level, we keep track of the satisfaction status of clauses as decoding proceeds, at each time step grouping candidates based on satisfied clauses, and selecting highest-scoring ones within top-value groups to fill in the next beam. 
%As a result, we constrain the search space to strings which satisfy given constraints. 
%\ximing{add Dominance Set from Multi-Objective Optimization }

\subsubsection{Tracking literals and clauses}
For each hypothesis in beam, we keep track of satisfaction status of literals and clauses. At the beginning nothing was generated, we mark all positive literals as unsatisfied and all negative literals as satisfied. A clause will be marked as satisfied once at least one of its literals are satisfied.

To efficiently track the occurrence of constrained word/phrase as generation proceeds, we keep track of matched partial prefix of each literal in ongoing generation by maintaining a pointer to its token(s). At the beginning, the pointer is set to head. At each time step, if next token generated matches the next token of the pointer, we advance the pointer forward, otherwise we set the pointer to head to abort the generation of this constraint. A special case is that next token generated doesn't match the next token of the pointer but matches the first token of the sequence, then the generation of this constraint restarts, and we set the pointer to the first token. If the pointer reaches the end, this constraint has been generated in decoded sentence, and we'll mark this literal as satisfied or unsatisfied depending on whether it's positive or negative, and update its clause status accordingly.

\subsubsection{Optimization}
At each time step t, the decoder model generates a distribution over all vocabulary $V$ for $k$ hypotheses in current beam, resulting in a candidate score matrix of size $k \times |V|$. Standard beam search fills in beam at time step t + 1 with candidates corresponding to the $k$ best scores. Our method, on the other hand, select $k$ best candidates that's both optimal in score and number of satisfied clauses.

Along with generating score matrix, we produce advanced constraint state for each candidate by updating the constraint state of its previous hypotheses based on its next-token extension. To ensure progress is made towards satisfying all constraints at the end, we discard the candidates whose next-token extension makes some clause impossible to satisfy in the following decoding step. This situation can happen when some clauses contain only negative literals, and the next-token extension completes the generation of all these negative literals.

Our next step is to select best candidates that maximizes both sequence score and number of satisfied clauses. If we plot the candidates as points in a coordinate whose x-axis is number of satisfied clauses, and y-axis is sequence score, the optimal candidates are at top-right corner, which corresponds to high sequence score and more satisfied clauses. Following this intuition, We use threshold pruning to reduce candidate set and only keep the ones around top-right. Concretely, we'll remove candidates whose score is not within top-$\alpha$ or whose number of satisfied clauses is not within top-$\beta$, where $\alpha$ and $\beta$ are tunable threshold.

Now, we'll select $k$ item from reduced candidate set to fill in the next beam. We group the candidates into buckets based on satisfied constraint clauses. Then we iteratively pick and remove candidate with highest score within each bucket in a round-robin fashion until all $k$ slot are filled. As a result, we preserve most likely sequence for each set of satisfied clauses in beam. This not only ensure progress is made towards optimizing proposed objective but also encourage exploring candidates which satisfy constraint clauses in different order.

In the end, we'll select the one with maximum likelihood from finished hypothesises which satisfy maximum number of constraint clauses as the final output. As a result, we end up with the optimal sequence among all strings satisfying given logical constraints.

%Please refer to figure 1 for detailed algorithm

==> section_v2/backups/3_model_1.tex <==
\makeatletter
\newcommand{\stx}[1]{\mathpalette\giusti@stx{#1}}
\newcommand{\giusti@stx}[2]{%
  \mbox{%
    \medmuskip=\thinmuskip
    \thickmuskip=\thinmuskip
    $\m@th#1#2$%
  }%
}
\makeatother
\input{fig/c_example}
%\input{fig/constraint_method_table}
\section{Our Method: NeuroLogic Decoding}
NeuroLogic Decoding generalizes past work by accepting any constraint in conjunctive normal form (CNF), which can represent any propositional logic formula. Our method efficiently leverages constraints 
% as prior knowledge 
to restrict the search space, leading to better generation quality. 

Sequence generation can be viewed as an optimization problem. The optimal output sequence $\hat{\textbf{y}}$ given input \textbf{x} is the one that maximizes the conditional probability $P_\theta(\textbf{y}|\textbf{x})$ parameterized by a model $\theta$
\[\hat{\textbf{y}} = \arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\]

Beam search \cite{Och2004TheAT} is an effective local search algorithm for finding approximately-optimal solution and has become the de-facto choice for generating sequences from conditional neural language models.
Sequence generation with lexical constraints can be viewed as a \textit{constrained} optimization problem, where the output space is restricted to only those sequences that satisfy the given constraints. We formalize the notation of logical constraints in section \ref{section: notation}, and present our proposed algorithm to find approximately-optimal solutions for constrained optimization in section \ref{section: algo}.

%\subsection{Notation} \label{section: notation}
%Predicate $D(\textbf{c})$ is a boolean function indicating whether a word or phrase $\textbf{c}$ occurs in a sequence $\textbf{y}$. $D(\textbf{c})$ will be true iff \textbf{y} contains $\textbf{c}$. Formally, 
%\begin{align*}
%    &D(\textbf{c}) \equiv \exists \: i, \> \textbf{y}_{i:i+|\textbf{c}|} = \textbf{c}
%\end{align*}
%For instance, enforcing a single positive or negative constraint $\textbf{c}_\textbf{i}$ to be satisfied is equivalent to enforcing literal $D(\textbf{c}_\textbf{i})$ or $\neg D(\textbf{c}_\textbf{i})$ to be true. Two or more single constraints can be connected using any logical operator to form a compound logical constraint $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ to represent arbitrarily complex lexical constraints. Table \ref{tab:c_examples} shows some examples. Previous works, on the other hand, only take constraints in certain form, which limits their expressiveness. 

%Our goal in this work is to find a way to enforce these logical constraints on generation output.
%Formally, we seek an optimal solution $\hat{\textbf{y}}$ for the following constrained optimization problem:
%\begin{align*}
%    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\\
%    &\text{subject to}\\
%    &D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n}) \text{ is true }
% \end{align*}
 
% \ximing{perhaps we will need to find a cleaner way to replace $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ to express compound constraint, thoughts/ideas ? }

\begin{figure*}[t]
\centering
    \includegraphics[width=1\linewidth]{fig/fig2_v5.pdf}
     \caption{Algorithm of selecting hypothesis to fill in next beam from candidates \rowan{we want to show the following 1. we can use a new constraint that has never been used before-- `Use at least one of X or Y', 2. we can do so without recomputing everything. 3. We want to have diversity in the satisfaction status (allowing for exploration) <- mention this at the beginning of the new sec3 To this, you might not need multiple rows or a multi-clause expression and putting it in natural language could help. For the $\alpha$/$\beta$ constraints maybe use a fake bar graph}
     } 
\end{figure*} 

\subsection{Algorithm} \label{section: algo}

\method accepts lexical constraints in Conjunctive Normal Form (CNF):
% Thus, it is sufficient to assume that all constraints our algorithm deals with are in CNF. 
% Without loss of generality, we assume that constraints $D(\textbf{c}_\textbf{0}, \cdots, \textbf{c}_\textbf{n})$ can be expressed in CNF:
\[\big(D_1 \lor D_2 \cdots \lor D_i \big) \land \cdots \land \big(D_k \lor D_{k+1} \cdots \lor D_n \big) \]
where each $D_i$ represents a single positive or negative lexical constraint  $D(\textbf{c}_\textbf{i})$ or $\neg D(\textbf{c}_\textbf{i})$ indicating word/phrase $\textbf{c}_\textbf{i}$ is strictly included or omitted (respectively). Any combination of such constraints that expressible as a predicate logical formula can be converted to CNF, and thus handled by \method. Notationally, we will refer to each individual constraint $D_i$ as a literal, and the disjunction of literals (bracketed AND term, above) as a clause, denoted as $C_j$, with N being the total number of clauses. Our method seeks optimal sequences in which all clauses are satisfied, formally 
\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x})\\
    &\text{subject to}\\
    & \sum_{i=1}^{N} C_i = N
 \end{align*}
Past work on constrained optimization introduces penalties \cite{Fiacco1976SensitivityAF} to approximate the constrained optimization problem with an unconstrained problem. Specifically, by adding a high-cost penalty term to the objective for violation of constraints:

\begin{align*}
    \hat{\textbf{y}} = &\arg\max_{\textbf{y} \in \mathcal{Y}}P_\theta(\textbf{y}|\textbf{x}) - \alpha' \sum_{i=1}^{N} C_i
 \end{align*}
where high $\alpha'$ results in significant objective reduction for any missing constraints. Intuitively, this objective aims to optimize both sequence likelihood (term 1) and number of satisfied clauses (term 2). 

We take a related approach, by attempting to find sequences that do well at both term 1 and term 2. While exhaustive search is intractable, we use a modified beam search to find approximately-optimal solutions for this objective. At each decoding step, we fill the beam with the most likely (term 1) candidates across a range of values for term 2, allowing a balance of candidates that are most likely, and satisfy the most constraints in each beam. In the end, we take the candidates with the most constraints satisfied (term 2), and select the most probable (term 1) one from this group. 
%As a result, we constrain the search space to strings which satisfy given constraints. 
%\ximing{add Dominance Set from Multi-Objective Optimization }

\subsubsection{Tracking literals and clauses}
For a clause $C_i$, if its satisfaction can not be violated in later decoding step, we say it is \emph{robustly satisfied}. A clause is \emph{robustly satisfied} if and only if at least one of its literals is satisfied positive literal.
%\[ C^i_{\textbf{y}_t} \textnormal { is true} \longrightarrow \forall \> t' > t, \: C^i_{\textbf{y}_{t'}} \textnormal { is true} \]
 On the other hand, if the satisfaction state of a clause $C_i$ can be violated by later generation, we refer to it as \emph{vulnerably satisfied}. This situation can happen when the clause has one or more satisfied negative literals, but no satisfied positive literal. 

At each time step for each hypothesis in beam, we keep track of its satisfaction status of literals and clauses. At the beginning when nothing has been generated, all positive literals are unsatisfied and all negative literals are satisfied. A clause will be marked as satisfied once at least one of its literals is satisfied. As decoding proceeds, we only need to keep track of unsatisfied clauses and \emph{vulnerably satisfied} clauses.

To efficiently track the occurrence of constrained word/phrase as generation proceeds, we keep track of matched partial prefix of each literal in ongoing generation by maintaining a pointer to its token(s). At the beginning, the pointer is set to head. At each time step, if next token generated matches the next token of the pointer, we advance the pointer forward, otherwise we set the pointer to head to abort the generation of this constraint. A special case is that next token generated doesn't match the next token of the pointer but matches the first token of the sequence, then the generation of this constraint restarts, and we set the pointer to the first token. If the pointer reaches the end, this constraint has been generated in decoded sentence, and we'll mark this literal as satisfied or unsatisfied depending on whether it's positive or negative, and update its clause status accordingly.

\subsubsection{Optimization}
At each time step t, the decoder model generates a distribution over all vocabulary $V$ for $k$ hypotheses in current beam, resulting in a candidate score matrix of size $k \times |V|$. Standard beam search fills in beam at time step t + 1 with candidates corresponding to the $k$ best scores. Our method, on the other hand, select $k$ best candidates that's both optimal in score and number of satisfied clauses.

Along with generating score matrix, we produce advanced constraint state for each candidate by updating the constraint state of its previous hypotheses based on its next-token extension. To ensure progress is made towards satisfying all constraints at the end, we discard the candidates whose next-token extension makes some clause impossible to satisfy in the following decoding step. This situation can happen when some clauses contain only negative literals, and the next-token extension completes the generation of all these negative literals.

Our next step is to select best candidates that maximizes both sequence score and number of satisfied clauses. If we plot the candidates as points in a coordinate whose x-axis is number of satisfied clauses, and y-axis is sequence score, the optimal candidates are at top-right corner, which corresponds to high sequence score and more satisfied clauses. Following this intuition, We use threshold pruning to reduce candidate set and only keep the ones around top-right. Concretely, we'll remove candidates whose score is not within top-$\alpha$ or whose number of satisfied clauses is not within top-$\beta$, where $\alpha$ and $\beta$ are tunable threshold.

Now, we'll select $k$ item from reduced candidate set to fill in the next beam. We group the candidates into buckets based on satisfied constraint clauses. Then we iteratively pick and remove candidate with highest score within each bucket in a round-robin fashion until all $k$ slot are filled. As a result, we preserve most likely sequence for each set of satisfied clauses in beam. This not only ensure progress is made towards optimizing proposed objective but also encourage exploring candidates which satisfy constraint clauses in different order and address the issue that .

In the end, we'll select the one with maximum likelihood from finished hypothesises which satisfy maximum number of constraint clauses as the final output. As a result, we end up with the optimal sequence among all strings satisfying given logical constraints.

%Please refer to figure 1 for detailed algorithm

==> section_v2/backups/4_experiment_0.tex <==

%Same with beam search, our method can be directly applied to any sequence decoding without requiring any modification of the model structure or training pipeline. We'll demonstrate the feasibility and flexibility of our method in various scenarios: constrained scene generation, cooking recipe generation, dialogue response generation, reducing gender bias in machine translation, and fine-grained image captioning. Additionally, we demonstrate the increase of controllablity brought by our method over pretrained language model in a zero-shot setting . 

\begin{center}
    \input{fig/result_comGen_model}
\input{fig/result_comGen_zeroshot}
\end{center}
\input{fig/result_comGen_decode}
\begin{figure*}[t]
\centering
    \includegraphics[width=1\linewidth]{fig/data_efficiency.png}
     \caption{Performance of GPT2-Large with respect to amount of training data, \textcolor{amber(sae/ece)}{orange line} denotes decoding with \textsc{NeuroLogic Decoding}, \textcolor{blue}{blue line} denotes decoding with vanilla beam search} \vspace{4mm}
    \includegraphics[width=1\linewidth]{fig/model_size.png}
     \caption{Performance of GPT2 with respect to model size, \textcolor{purple}{purple line} and \textcolor{yellow}{yellow line} denotes decoding with and without \textsc{NeuroLogic Decoding} in in supervised setting, \textcolor{darkblue}{dark line} denotes decoding with \textsc{NeuroLogic Decoding} in zero-shot setting} 
\end{figure*} 
\begin{figure}[t]
\centering
    \includegraphics[width=1\linewidth]{fig/examples.pdf}
     \caption{A generation example of different models in supervised and zero-shot setting with and without \textsc{NeuroLogic Decoding}} 
\end{figure} 

\section{Experiments}
\subsection{Constrained scene generation}
C{\small OMMON}G{\small EN} is a benchmark dataset, explicitly testing generative commonsense reasoning. Given a set of common concepts (e.g., {dog, frisbee, catch, throw}); the task is to generate a coherent sentence describing an everyday scenario using these concepts (e.g., “a man throws a frisbee and his dog catches it”)

\paragraph{Problem Formulation} The input is an unordered set of $k$ concepts $x = \{c_1, c_2, \ldots , c_k\}$, where each concept $c_i \in \mathcal{C}$ is a common object (noun) or action (verb). The expected output is a simple, grammatical sentence $y \in \mathcal{Y}$ that describes a common scenario  using all given concepts in $x$ with correct morphological inflections. 

To apply NeuroLogic Decoding, we impose that each $c_i$ must appear in output $y$ under some morphological inflection. For each given concept $c_i$, let $M_i = \{m^i_1, \ldots m^i_{|M_i|}\}$ denote all possible inflections of $c_i$. If output $y$ covers concept $c_i$, then at least one of $\{m^i_1, \ldots m^i_{|M_i|}\}$ must appear in $y$. Formally, 
\[\forall \> c_i \in x,\> \exists \> m^i_{j} \in M_i,\> \mathcal{D}(m^i_{j})\]
where $\mathcal{D}(m_{ij}$ is a boolean-value function indicating whether $\textbf{y}$ contains $m_{ij}$ or not, as defined above. The equivalent predicate logical expression is 
\begin{align*}
    \Big(D(m^1_1) \lor  \ldots \lor D(m^1_{|M_1|})\Big) \land \ldots\\
    \land \Big(D(m^k_1) \lor \ldots \lor D(m^k_{|M_k|}) \Big) 
\end{align*}
\begin{align*}
     \bigwedge\limits_{i=1}^k \Big( \bigvee_{j=1}^{|M^i|} D(m^i_j)\Big)
\end{align*}
\paragraph{Dataset}
C{\small OMMON}G{\small EN} dataset consisting of 29,599 concept-sets (train 27,069, val 993, test 1,497) associated with 49,129 sentences. The average size of concept-sets in test set is 4.5. There are on average four sentences for each concept-set. The average length of the sentence is 13.8 . 
\paragraph{Approach and Baseline}
We consider C{\small OMMON}G{\small EN} as a conditional sentence generation task. Since there's no proposed method for C{\small OMMON}G{\small EN} setting yet, the comparison is between generation using seq2seq language models with vanilla beam decoding, with previous constrained decoding, and with proposed logical constrained decoding. The seq2seq models we consider includes GPT-2  \cite{radford2019language}, UniLM \cite{NIPS2019_9464}, UniLM-v2 \cite{bao2020unilmv2}, BERT-Gen \cite{bao2020unilmv2}, BART \cite{lewis-etal-2020-bart}, and T5 \cite{raffel2019exploring}. All models are finetuned with their default hyperparameters. 
\paragraph{Results}
Table \ref{tab:comGen_result} presents the experimental results of all compared methods in different metrics. We can see that for all language models, decoding with our logical constraints outperforms decoding with beam search, sampling method and previous constraint method in all metric with a significant margin. With UniLM, we reach new SOTA results on C{\small OMMON}G{\small EN} without requiring any modification of the model structure or training pipeline. Our performance gain comes from better search space by incorporating lexical prior as logical constraints. Previous constraint methods, on the other hand, fail to handle morphological cases and suffer from significant performance drop on generation quality.

\subsubsection{Zero-shot scene generation}
Large-scale pre-trained language models have shown promising language generation capabilities, however besides initial prompt there's little or no controllability over the language content. On the other hand, with our constrained decoding, we can force any language models to generate sentences satisfying given constraints. We leverage such ability to generate plausible scenes involving given concepts with pre-trained LM in zero-shot setting. We believe that due to the massive pre-training, pre-trained LM possess the underlying knowledge of given concepts and understanding of commonsense relations between concepts. What we need to do is to retrieve a globally optimal scenario composed by all given concepts in decoding phrase. We achieve such retrieval via proposed constrained decoding. 
%understand given concepts and associate given concepts with suitable intersection.

The pre-trained language models we examine in zero-shot constrained generation includes GPT \cite{Radford2018ImprovingLU}, GPT-2 \cite{radford2019language}, Transformer XL \cite{dai-etal-2019-transformer}, and CTRL \cite{keskar2019ctrl}.

%\input{fig/zero_shot_comGen}
%\input{fig/result_zero_shot}

\paragraph{Results} 
Table \ref{tab:zero_com} demonstrates some examples generated by GPT2 with proposed constrained decoding. We can see that these examples are grammarly correct and commonsensically reasonable, although their text style differ from caption language in target set.  

Because the style and domain of generated sentences varies a lot depending on used pretrained language model, automatic evaluation metric against groudtruth output would be poor indicator for language quality and commonsensical rationality. Instead, we conduct human evaluation on generation quality, crowd sourcing on Amazon Mechanical Turk. We ask turker whether given sentence is semantically valid and commonsensically valid. For instance, 'A dog is walking a man on the sidewark' conveys valid semantic meaning but violates commonsense fact. We conduct such evaluation over 100 examples from our test set for each LM. Table \ref{tab:zero_result} shows the human eval results. 

%\item performance gain by fine-tuning indicating increase of reasoning ability or just a result of language domain adaption?
%\item correlation of performance with the strength of LM ?
\input{fig/result_recipe}
\subsection{Cooking recipe generation}
The second task is cooking recipe generation. Given a recipe title (i.e., the name of the dish), and the list of ingredients, the task is to generate the correct cooking instructions for given recipe. 

\paragraph{Problem Formulation}  The input is recipe title, an unordered set of ingredients $E = \{e_1, ..., e_{|E|}\}$ where each $e$ can be a single- or multi-word ingredient phrase (e.g., 'onions', 'black pepper'). Let $\mathcal{G}$ denote the set of all ingredients. The expected output is a paragraph $y \in \mathcal{Y}$ that describes multi-step cooking instruction.  

The lexical constraint here is that all given ingredients $e_i$ must appear in instruction $y$ and all other ingredients $\mathcal{G} - E$ must not appear. It can be the case that instruction $y$ uses generic term to refer ingredients. (i.e. 'onions', 'green beans', 'carrot' are considered covered if y contains 'vegetables')  Denotes the generic name for ingredient $e_i$ as $e^T_i$. Formally, lexical constraint is 
\[\Big(\forall \> e_i \in E,\> \mathcal{D}(e_i) \lor \mathcal{D}(e^T_i)\Big) \land \Big(\forall \> e_i \in \mathcal{G} - E, \neg \mathcal{D}(e_i)\Big ) \]
\paragraph{Dataset} We use Recipe1M+ dataset. There are about 111,567 recipes in total (train 109,567, val 1,000, test 1,000). We exclude the recipes whose instructions have less than 10 tokens or more than 500 tokens, those recipes take about 0.1\% of all data set. On average each recipe has 118 tokens and 9 ingredients.
\paragraph{Approach and Baseline} We view recipe generation as conditional sentence generation task, and generates using seq2seq language models with proposed constrained decoding. The seq2seq models we consider includes GPT-2  \cite{radford2019language}, UniLM \cite{NIPS2019_9464}, BART \cite{lewis-etal-2020-bart}, and T5 \cite{raffel2019exploring}. All models are finetuned with their default hyperparameters. 
We include three previous work on recipe generation as baselines \cite{kiddon-etal-2016-globally, bosselut-etal-2018-discourse, yang-etal-2017-reference}. Moreover, we compare with performance of seq2seq language models considered above with vanilla beam decoding as additional baselines. 

\paragraph{Result} Table \ref{tab:result_recipe} presents the experimental results. We can see that our approach outperform all baselines in all metrics. With BART, we reach new SOTA results. The biggest improvement is on coverage of given ingredients and usage of extra ingredients. With proposed decoding algorithm, we're able to cover almost all ingredients in generated instructions and guarantee not to use any other ingredients, which leads to more controllable recipe generation.

\input{fig/result_dialogue}
\subsection{Dialogue response generation}

The third task is dialogue responses generation for hotel and restaurant information systems from \cite{wen-etal-2016-multi}. The task is to generate a natural language response given a query type (e.g., informing or querying) and a list of facts to convey (e.g., a hotel’s name and address). 
\paragraph{Problem Formulation} 
The input is query type, unordered set of facts $F = \{f_1, ..., f_{|F|}\}$, where each $f_i$ contains attribute and value (i.e. accepts\_credit\_cards=”yes”, name=”red victorian bed breakfast”). The expected output is a dialogue responses $y \in \mathcal{Y}$ containing given information. 

The lexical constraint here is that all given facts $f_i$ must be included in responses $y$ in proper nature language form $f^N_i$. For attribute with boolean value only, $f^N_i$ is the attribute or negation of the attribute depending on its value, otherwise $f^N_i$ is the value itself. Formally,
\[\forall \> f_i \in F,\> \mathcal{D}(f^N_i)\]


\paragraph{Dataset} We used the hotel and restaurant dialogue system corpus and the same train-development-test split from Wen et al. (2015). There are 8 system dialogue act types and 12 types of attributes.

\paragraph{Approach and Baseline}
We view dialogue response generation as conditional sentence generation task, and generates using seq2seq language models with proposed constrained decoding. The seq2seq models we consider includes GPT-2  \cite{radford2019language}, UniLM \cite{NIPS2019_9464}, BART \cite{lewis-etal-2020-bart}, and T5 \cite{raffel2019exploring}. All models are finetuned with their default hyperparameters. 
We include three previous work on dialogue response generation as baselines \cite{kiddon-etal-2016-globally, bosselut-etal-2018-discourse, yang-etal-2017-reference}. Moreover, we compare with performance of seq2seq language models considered above with vanilla beam decoding as additional baselines. 
\paragraph{Result}
Table \ref{tab:comGen_result} presents the experimental results. We can see that our approach outperform all baselines in all metrics. With GPT-2, we reach new SOTA results. 
%\subsubsection{Zero-shot dialogue generation}
%\ximing{This task is easy, might only keep the zero-shot setting and skip superivised}

\input{fig/result_gender}
\subsection{Reducing gender bias}
 Learned models exhibit social bias when their training data encode stereotypes. In the many languages which associate between biological and grammatical gender, the gender of an animate object can be identified via morphological markers. In fact, many MT systems, such as Google Translate or Microsoft Translator exhibit biases, e.g., translating nurses as females and programmers as males, regardless of context. We aim to reduce such bias via constraint decoding. 


\paragraph{Problem Formulation} 
The input $x$ is an English sentence describes a scenario with human entities $N = \{n_1, \ldots, n_{|N|}\}$ who are identified by their role. Expected output is a translation $y$ which use correct gender inflection in target-language $L$. The only indicator for gender information in English is pronoun. Through co-reference resolution \cite{lee-etal-2017-end}, we can associate pronoun with its corresponding human entity. 

The lexical constraint here is that human entity resolved to gender-specific pronoun much appear with correct gender inflection in output $y$. For a human entity $n_i$, let $n^F_i$ denotes its female inflection in target-language $L$, and $n^M_i$ denotes its female inflection. Let $F$ denotes set of human entities associated with female character, let $M$ denotes set of entities associated with male. Formally, the lexical constraint is 
\begin{align*}
    \Big(\forall n_i \in F,\mathcal{D}(n^F_i) \land \neg \mathcal{D}(n^M_i)\Big) \land \\
    \Big(\forall n_i \in M,\mathcal{D}(n^M_i) \land \neg \mathcal{D}(n^F_i) \Big) 
\end{align*}

\paragraph{Dataset} We use the same dataset with \cite{stanovsky-etal-2019-evaluating}, which is introduced by two recent coreference gender-bias studies: the Winogender and the Wino-Bias datasets.
\paragraph{Approach and Baseline} We test 3 MT models with and without constraint decoding. 1) the model of \cite{ott-etal-2018-scaling}, which achieved the best performance on English-to-French translation on the WMT’14 test set. 2) the model of \cite{edunov-etal-2018-understanding}, the WMT’18 winner on English-to-German translation. and 3) Large-scale pretrained language model T5 \cite{raffel2019exploring} with control code on English to German, French, and Romanian translation. 
We compare the performance of these MT models with and without constraint decoding. 

\paragraph{Result} We can see that proposed constraint decoding boosts overall gender accuracy (\% of instances the translation had the correct gender) of all MT systems without requiring any additional training or modification on training dataset. 

%\subsection{fine-grained image captioning}
%\include{fig/result_caption}


%\section{Ablation}
%We conduct ablations to study 1) the compatibility of our method with various seq2seq model 2) the effect of bucket key on different tasks. 
%\subsection{Backbone seq2seq model}
%\subsection{Bucket key}
